Changes in air quality and human mobility in the U.S. during the COVID-19 pandemic

The first goal of this study is to quantify the magnitude and spatial variability of air quality changes in the US during the COVID-19 pandemic. We focus on two federally regulated pollutants, nitrogen dioxide (NO2), and fine particulate matter (PM2.5). Observed concentrations at all available ground monitoring sites (240 and 480 for NO2 and PM2.5, respectively) were compared between April 2020 and April of the prior five years, 2015-2019, as the baseline. Large statistically significant decreases in NO2 concentrations were found at more than 65% of the monitoring sites, with an average drop of 2 ppb when compared to the mean of the previous five years. The same patterns are confirmed by satellite-derived NO2 column totals from NASA OMI. PM2.5 concentrations from the ground monitoring sites, however, were more likely to be higher. The second goal of this study is to explain the different responses of the two pollutants during the COVID-19 pandemic. The hypothesis put forward is that the shelter-in-place measures affected peoples' driving patterns most dramatically, thus passenger vehicle NO2 emissions were reduced. Commercial vehicles and electricity demand for all purposes remained relatively unchanged, thus PM2.5 concentrations did not drop significantly. To establish a correlation between the observed NO2 changes and the extent to which people were sheltering in place, we use a mobility index, which was produced and made public by Descartes Labs. This mobility index aggregates cell phone usage at the county level to capture changes in human movement over time. We found a strong correlation between the observed decreases in NO2 concentrations and decreases in human mobility. By contrast, no discernible pattern was detected between mobility and PM2.5 concentrations changes, suggesting that decreases in personal-vehicle traffic alone may not be effective at reducing PM2.5 pollution.

==> Introduction.tex <==

Worldwide, about 91\% of the population is exposed to poor air quality. The World Health Organization (WHO) estimates that on average, 4.2 million people die each year from causes directly attributed to air pollution \cite{whodeath}. Nitrogen dioxide (\ce{NO2}) is one of a group of highly reactive gases known as nitrogen oxides (\ce{NOx}). \ce{NO2} can irritate the human respiratory system and is also harmful to ecosystems by the formation of nitric acid and acid rain \cite{epano2,lin2011}. \ce{PM_{2.5}} is another harmful air pollutant that consists of microscopic particles with a diameter smaller than 2.5 $\mu$m. These particles can pose a great risk to human health because they can penetrate into human lungs and even the bloodstream; \ce{PM_{2.5}} is also often associated with poor visibility \cite{epapm}. \ce{NO2} and \ce{PM_{2.5}} are both primary (i.e., they can be directly emitted into the atmosphere) and secondary (i.e., they can also form after chemical reactions in the atmosphere) pollutants. High concentrations of both are not necessarily found where their emissions are highest, due to processes such as chemical reactions, transport, or diffusion. \ce{NO2} and \ce{PM_{2.5}} are the main focus of this paper because they are among the seven ``criteria" pollutants that are regulated at the federal level by the U.S. Environmental Protection Agency (EPA) via the National Ambient Air Quality Standards (NAAQS). %The other five criteria pollutants are: lead, ozone, particulate matter of 10 $\mu m$ in diameter (\ce{PM_{10}}), carbon monoxide (\ce{CO}), and sulfur dioxide (SO2). 

The novel coronavirus disease (SARS-CoV-2/COVID-19, COVID-19 hereafter for brevity) was first identified in Wuhan, China, on December 30, 2019 \cite{who,chan2020}. Cases started to spread initially in China but quickly expanded to other countries across the world. COVID-19 was declared a global pandemic in March 2020 \cite{whoEurope}. At the time of this study, over 9 million people have been affected by the virus, with over 470,000 deaths in 213 countries and territories \cite{worldometer,JHU}. COVID-19 first reached the U.S. in February 2020 and since then it has caused over 120,000 deaths in the span of a few months \cite{cdc,JHU}. The death rate of COVID-19 is significantly higher among people with cardiovascular and respiratory illnesses \cite{acc}, which are also strongly connected with air pollution \cite{isaifan2020}. Furthermore, new studies suggest that higher concentrations of air pollutants result in a higher risk of COVID-19 infection \cite{yongjian2020} and mortality \cite{wu2020}.

In the U.S., social distancing measures were implemented state by state with the goal of limiting the spread of the pandemic. In general, closure or non-physical interaction options (e.g., delivery only) were implemented for schools, restaurants, and public places of gathering. Businesses, workers, and types of activities that were deemed essential during the pandemic either continued operating under strict protection measures (e.g., personal protective equipment (PPE), masks) or switched to online work. Non-essential businesses requiring physical presence and interaction closed completely (e.g., hair salons, bars, gyms). The extent of social distancing measures, seriousness of the implementation, and the degree of compliance varied throughout the U.S. Most states announced some level of social distancing orders starting in mid-March, 2020 \cite{bbc}, often including a mandatory quarantine for people diagnosed with or showing symptoms of the coronavirus. By the beginning of April, almost all states had a mandatory shelter-in-place or lockdown order \cite{nystats}. Hereafter, lockdown and shelter-in-place will be used interchangeably. The social distancing measures have led to drastic changes in mobility and energy use and therefore changes in emissions of pollutants. 

Globally, the COVID-19 outbreak is forcing large changes in economic activities \cite{NCAR}. In China, following the strict social distancing measures, transportation decreased noticeably and, as a result, China experienced a drastic decrease in atmospheric pollution, specifically \ce{CO} \cite{NCAR}, \ce{NO2}, and \ce{PM_{2.5}} \cite{manuel2020,NCAR,nasa} concentrations in major urban areas. However, emissions from residential heating and industry remained steady or slightly declined \cite{chen2020}. Using satellite data, Zhang et al. \cite{zhang2020nox} and the National Center for Atmospheric Research \cite{NCAR} reported a 70\% and 50\% decrease in \ce{NOx} concentrations in Eastern China, respectively. Bao and Zhang \cite{bao2020} showed an average of 7.8\% decrease in the Air Quality Index over 44 cities in northern China. Bawens et al. \cite{Bauwensetal2020} and Shi and Brasseur \cite{ShiBra20} reported an increase in \ce{O3} concentrations in the same region. Chen et al. \cite{chen2020}, reported that \ce{NO2} and \ce{PM_{2.5}} concentrations were decreased by 12.9 and 18.9 $\mu$g/m$^3$, respectively. They estimated that this improvement in the air quality of China avoided over 10,000 \ce{NO2}- and \ce{PM_{2.5}}-related deaths during the pandemic, which could potentially outnumber the confirmed deaths related to COVID-19 in China \cite{chen2020}. Other researchers also have proposed that the improvements of air quality during the pandemic might have saved more lives than the coronavirus has taken \cite{dutheil2020,gfeed}. Likewise, Isaifan \cite{isaifan2020} argues that the shutting down of industrial and anthropogenic activities caused by COVID-19 in China may have saved more lives by preventing air pollution than by preventing infection.

European countries, such as France and Italy, experienced a sharp reduction in their air pollution amid COVID-19 \cite{esa}. In Brazil, a significant decrease in \ce{CO} concentrations and, to a lower extent, in \ce{NOx} levels was observed, while ozone levels were higher due to a decrease in \ce{NOx} concentrations in \ce{VOC}-limited locations \cite{dantas2020,nakada2020}. The same findings were observed in Kazakhstan and Spain, respectively \cite{kerimray2020,tobias2020changes}. Likewise, Iran \cite{nemati2020} and India \cite{mahato2020,sharma2020} reported noticeable improvements in air pollution during the pandemic. Le et al. \cite{le2020} looked into the impacts of the forced confinement on \ce{CO2} emissions and concluded that global \ce{CO2} emissions decreased by 17\% by early April compared to the average level in 2019. They believe that the yearly-mean \ce{CO2} emissions would decrease by 7\% if restrictions remain by the end of 2020.

In the United States, as a result of social distancing, states started to experience a dramatic decrease in personal transportation and mobility in general \cite{gao2020}. Personal vehicle transportation decreased by approximately 46\% on average nationwide, while freight movement only decreased by approximately 13\% \cite{inrixtraffic}. Air traffic decreased significantly as well \cite{businessinsider}. On-road vehicle transportation is a main source of \ce{NOx} emissions \cite{nei}. Airports too are usually hot spots for \ce{NO2} pollution \cite{nasa}.

The Houston Advanced Research Center (HARC) \cite{harc} analyzed the daily averages of hourly aggregated concentrations of benzene, toluene, ethylbenzene, and xylenes (BTEX) across six stations in Houston, USA. They reported a decrease in BTEX levels in the atmosphere while an intensified formation on \ce{PM_{2.5}} in the region. Similarly, the New York Times reported huge declines in pollution over major metropolitan areas, including Los Angeles, Seattle, New York, Chicago, and Atlanta using satellite data \cite{NYtimes}.

While a noticeable number of studies have looked into the correlation between lockdown measures amid COVID-19 and air quality in different countries, none has evaluated air quality for the entire United States. The goals of this study are to investigate the magnitude and spatial variability of air quality (\ce{NO2} and \ce{PM_{2.5}}) changes in the U.S. during the COVID-19 pandemic and to understand the relationships between mobility and \ce{NO2} changes. An innovative aspect of this study is that we use an extensive database of ground monitoring stations for \ce{NO2} and \ce{PM_{2.5}} (Section \ref{sec:AQdata}) and a third-party high-resolution mobility dataset derived from cellular device movement (Section \ref{sec:mob}). In addition, we included satellite-retrieved \ce{NO2} information to increase the spatial data coverage (Section \ref{sec:sat}). Whereas most studies rely only on a comparison to 2019, we consider five prior years (2015--2019) to provide a more robust measure.

